MoPEFT: A Mixture-of-PEFTs for the Segment Anything Model

The emergence of foundation models, such as the Segment Anything Model (SAM), has sparked interest in Parameter-Efficient Fine-Tuning (PEFT) methods that tailor these large models to application domains outside their training data. However, different PEFT techniques modify the representation of a model differently, making it a non-trivial task to select the most appropriate method for the domain of interest. We propose a new framework, Mixture-of-PEFTs methods (MoPEFT), that is inspired by traditional Mixture-of-Experts (MoE) methodologies and is utilized for fine-tuning SAM. Our MoPEFT framework incorporates three different PEFT techniques as submodules and dynamically learns to activate the ones that are best suited for a given data-task setup. We test our method on the Segment Anything Model and show that MoPEFT consistently outperforms other fine-tuning methods on the MESS benchmark.

==> 4_tables.tex <==
\begin{table*}
    \centering
    \begin{tabular}{|l|l|l|l|l|l|}
    \hline
        \textbf{Datasets} & \textbf{L=5} & \textbf{L=10} & \textbf{L=20} & \textbf{L=25} & \textbf{Baseline} \\
        \hline
        iSAID \cite{a} & 62.14 & 63.14 & 68.29 & 64.18 & 62.59 \\
        ISPRS Postdam \cite{a} & 28.92 & 29.92 & 40.42 & 37.94 & 29.73 \\ 
        WorldFloods \cite{a} & 46.75 & 48.75 & 63.17 & 64.02 & 46.45 \\
        FloodNet \cite{a} & 39.94 & 40.94 & 50.01 & 51.22 & 39.72 \\
        UAVid \cite{a} & 58.12 & 60.96 & 71.10 & 68.72 & 60.19 \\
        Kvasir-Instrument \cite{a} & 43.35 & 48.32 & 71.92 & 70.04 & 46.82 \\
        CHASE DB1 \cite{a} & 25.20 & 25.95 & 42.49 & 43.11 & 23.56 \\ \hline
    \end{tabular}
    \caption{Effect of Prefix Length on task performance}
\end{table*}

\begin{table*}[!htbp]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|}
    \hline
        \textbf{Adapters} & \textbf{$D_{mid}=48$} & \textbf{$D_{mid=64}$} & \textbf{$D_{mid}=128$} & \textbf{$D_{mid}=256$} & \textbf{Baseline} \\ \hline
        iSAID \cite{a} & 59.02 & 60.38 & 64.03 & 68.29 & 62.59 \\
        ISPRS Postdam \cite{a} & 19.23 & 23.44 & 35.03 & 40.42 & 29.73 \\
        WorldFloods \cite{a} & 13.01 & 42.82 & 51.29 & 63.17 & 46.45 \\
        FloodNet \cite{a} & 21.39 & 37.01 & 43.68 & 50.02 & 39.72 \\
        UAVid \cite{a} & 10.43 & 59.11 & 64.82 & 71.12 & 60.19 \\
        Kvasir-Instrument \cite{a} & 38.41 & 48.22 & 59.31 & 71.92 & 46.82 \\
        CHASE DB1 \cite{a} & 16.74 & 23.95 & 34.69 & 42.49 & 23.56 \\
        CryoNuSeg \cite{a} & 32.21 & 39.92 & 44.20 & 59.88 & 38.06 \\ \hline
    \end{tabular}
    \caption{Effect of bottleneck size on task performance}
\end{table*}
